Using Causality to Infer Coordinated Attacks in Social Media

The rise of social media has been accompanied by a dark side with the ease of creating fake accounts and disseminating misinformation through coordinated attacks. Existing methods to identify such attacks often rely on thematic similarities or network-based approaches, overlooking the intricate causal relationships that underlie coordinated actions. This work introduces a novel approach for detecting coordinated attacks using Convergent Cross Mapping (CCM), a technique that infers causality from temporal relationships between user activity. We build on the theoretical framework of CCM by incorporating topic modelling as a basis for further optimizing its performance. We apply CCM to real-world data from the infamous IRA attack on US elections, achieving F1 scores up to 75.3% in identifying coordinated accounts. Furthermore, we analyse the output of our model to identify the most influential users in a community. We apply our model to a case study involving COVID-19 anti-vax related discussions on Twitter. Our results demonstrate the effectiveness of our model in uncovering causal structures of coordinated behaviour, offering a promising avenue for mitigating the threat of malicious campaigns on social media platforms.

==> limitations.tex <==
puga

==> motivation.tex <==


We simulated two users $u_1$ and $u_2$ to simulate follower-following behaviour, which is a basic coordination strategy. We applied CCM to different types of simulations to observe cross map prediction accuracy measured with correlation at different library lengths. Figure \ref{fig:sim_1}, \ref{fig:sim_2}, \ref{fig:sim_3}, and \ref{fig:sim_4} shows our results for simulations. The increasing nature of correlation when there is a follower-following behaviour motivated us to adopt CCM to apply on real online social network (OSN) data. 

==> preliminaries.tex <==
We refer to an interaction made by a user with the OSN as an \emph{event}. For example, on Twitter (X) platform, a tweet authored by a user is considered an event. The set of timestamps of events authored by a user $u$ is called an activity trace $\{t_{0,u}, t_{1,u}, \dots\}$. If there is an influence flow from user $u_1$ to $u_2$, we say $u_1 \Rightarrow u_2$. If $u_1 \Rightarrow u_2$ and $u_2 \Rightarrow u_1$, we say there is a bidirectional coupling. If $u_1 \Rightarrow u_2$ but $u_1 \nRightarrow u_2$, we say that there exists a unidirectional coupling.

